Non-Reciprocal yet Equilibrium Critical Dynamics

Non-reciprocal interactions find broad applicability in non-equilibrium and living systems. Their canonical implementation involves asymmetric couplings between two entities, which generally induce spatio-temporal patterns and time-dependent steady states that break time-translational invariance, representing a clear deviation from equilibrium physics. Although their phenomenology is well understood, whether non-reciprocal interactions induce new universality classes, and if so, under what conditions, remains an open question. In the present work, we perform a field-theoretic renormalization group (RG) analysis of the dynamics of two non-reciprocally coupled $n$-vector order parameters possessing a $U(n)$ symmetry, generalizing previous results to order parameters with multiple components, a feature that has been shown to generate novel non-equilibrium critical behavior in certain non-reciprocal systems. To lowest order in $\epsilon = 4-d$, we find that the non-reciprocal coupling is RG-irrelevant, and the critical behavior is governed by the equilibrium fixed point of the Model A universality class of Hohenberg and Halperin with $2n$ vector components, even though the transition is into a non-equilibrium state. Our results demonstrate that non-reciprocity alone may not be sufficient to induce novel universality classes.

==> feynmanD.tex <==
\newcommand{\noisediagram}[1][0.3]{%
  \scalebox{#1}{\begin{tikzpicture}[baseline = (o.base)]
  \begin{feynman}
    \vertex (a) at (0,0) ;
    \vertex (b) at (0.4,0) ;
    \vertex (c) at (0.8,0);
    \vertex [above left=of a] (o1) ;
    \vertex [below left=of a] (o2) ;
    \vertex (a1) at ($(a)!0.7!(o1)$);
    \vertex (a2) at ($(a)!0.7!(o2)$);
    % First curve with moderate bend
    \diagram* {
      (a1) -- [anti propagator] (a),
      (a1) -- [propagator] (b),
      (a1) -- [propagator] (c),
      (a2) -- [propagator] (a),
      (a2) -- [anti propagator] (b),
      (a2) -- [anti propagator] (c),
    };
  \end{feynman}
\end{tikzpicture}%
}
}

\newcommand{\diffdiagramone}[1][0.3]{%
  \scalebox{#1}{\begin{tikzpicture}[baseline = (o.base), scale = 1.4]
\begin{feynman}
\vertex (o) at (0,0);
\vertex (a1) at (0.4,0);
\vertex (a2) at ($(a1) + (1,0)$);
\vertex (a3) at ($(a2) + (0.33,0.5)$);     % 1 unit above a
\vertex (a4) at ($(a2) + (0.33,-0.5)$);    % 1 unit below a
\vertex (i) at ($(a2) + (1,0)$);  % relative to b
\diagram* {
(a1) -- [propagator] (a2),
(a1) -- [propagator] (a3),
(a2) -- [anti propagator] (a3),
(a1) -- [anti propagator] (a4),
(a2) -- [propagator] (a4),
};
\end{feynman}
\end{tikzpicture}%
}
}

\newcommand{\diffdiagramtwo}[1][0.3]{%
  \scalebox{#1}{\begin{tikzpicture}[baseline = (o.base), scale = 1.4]
\begin{feynman}
\vertex (o) at (0,0);
\vertex (a1) at (0.4,0);
\vertex (a2) at ($(a1) + (1,0)$);
\vertex (a3) at ($(a2) + (0.33,0.5)$);     % 1 unit above a
\vertex (a4) at ($(a2) + (0.33,-0.5)$);    % 1 unit below a
\vertex (i) at ($(a2) + (1,0)$) {\(b\)};  % relative to b
\diagram* {
(a1) -- [anti propagator] (a2),
(a1) -- [propagator] (a3),
(a2) -- [anti propagator] (a3),
(a1) -- [propagator] (a4),
(a2) -- [anti propagator] (a4),
};
\end{feynman}
\end{tikzpicture}%
}
}

